Deep Lifetime Clustering

The goal of lifetime clustering is to develop an inductive model that maps subjects into $K$ clusters according to their underlying (unobserved) lifetime distribution. We introduce a neural-network based lifetime clustering model that can find cluster assignments by directly maximizing the divergence between the empirical lifetime distributions of the clusters. Accordingly, we define a novel clustering loss function over the lifetime distributions (of entire clusters) based on a tight upper bound of the two-sample Kuiper test p-value. The resultant model is robust to the modeling issues associated with the unobservability of termination signals, and does not assume proportional hazards. Our results in real and synthetic datasets show significantly better lifetime clusters (as evaluated by C-index, Brier Score, Logrank score and adjusted Rand index) as compared to competing approaches.

==> dataset.tex <==
%!TEX root = paper.tex
\section{Dataset} \label{sec:dataset}
 %\bruno{Need to significantly compact this section DONE}
In this paper, we analyze a large-scale social network dataset collected from Friendster. 
%Friendster was founded in 2002 and was one of the earliest social networking websites, reaching 3 million users within the first few months \citep{friendsterstats}. The website allowed users to share messages, photos and videos with other members.
After processing 30TB of data, originally collected by the Internet Archive in June 2011, the resulting network has around 15 million users with 335 million friendship links. Each user has profile information such as age, gender, marital status, occupation, and interests. Additionally, there are user comments on each other's profile pages with timestamps that indicate activity in the site. %See Table \ref{tab:dataset} for some additional statistics on the dataset. 
We have made our processed data available to the public at \textit{location} (anonymized).

%\begin{table}[h!]
%\centering
%\begin{tabular}{|c|c|}
%\hline
%\# Users & 15M\\
%\hline
%\# Friendship links & 335M\\
%\hline
%\# Comments & 75M\\
%\hline
%\# Users with atleast one comment & 9.5M\\
%\hline
%\# Users with atleast ten comments & 1.93M\\
%\hline
%\# Users with Age, Gender \& Location specified & 6.47M\\
%\hline
%\end{tabular}
%\caption{Statistics on the Friendster dataset}
%\label{tab:dataset}
%\end{table}


In our experiments, we only use the data up to March 2008 as Friendster was shown to face continuous decline since then because of the introduction of ``new Facebook wall'' \citep{brunowsdm}. From this, we only consider a subset of 1.1 million users who had participated in at least one comment, and had specified their basic profile information like age and gender. 

We build the dataset $\mathcal{D} : \{X_u, \{Y_{u, i}\}_{i=1}^{q_u}, S_u\}$ (Definition~\ref{def:dataset}) for our clustering task as follows. \\
$X_u$ : We use each user's profile information (like age, gender, relationship status, occupation and location) as features. To help improve the performance of competing methods, we also construct additional features using the user's activity over the initial months (like number of comments sent and received, number of individuals interacted with, etc.). \\
%construct around 60 features for each user $u$ in the Friendster dataset using the profile information (like age, gender, relationship status, occupation and location), and using the user's activity over the initial months (like number of comments sent and received, number of individuals interacted with, etc.).\\
$Y_{u, i}$ : We define $Y_{u, i}$ as the time between $u$'s $i$th comment (sent or received) and $(i-1)$st comment (sent or received). $q(u)$ is then defined as the total number of comments the user participated in. \\
$S_u$ : We calculate $S_u$ as the time between $u$'s last activity and the chosen time of measurement (March 2008). 

%\cite{brunowsdm} depicted the effect of the introduction of ``new Facebook wall'' in July 2008 to other competing social networking websites including Friendster. It is clear from their analysis that Friendster faced a continuous decline in the number of daily active users since then. Seeing that we wish to analyze the system on its own without any external influence, we only use the data upto March 2008 (six years from the introduction of Friendster) and disregard the rest. 

